Principal Component Analysis with Tensor Train Subspace

Tensor train is a hierarchical tensor network structure that helps alleviate the curse of dimensionality by parameterizing large-scale multidimensional data via a set of network of low-rank tensors. Associated with such a construction is a notion of Tensor Train subspace and in this paper we propose a TT-PCA algorithm for estimating this structured subspace from the given data. By maintaining low rank tensor structure, TT-PCA is more robust to noise comparing with PCA or Tucker-PCA. This is borne out numerically by testing the proposed approach on the Extended YaleFace Dataset B.

==> Algo_TTNPE.tex <==
\begin{algorithm}
   \caption{Tensor Train Neighbor Preserving Embedding (TT-NPE) Algorithm}
   \begin{algorithmic}[1]
   \INPUT  $N$ tensors $\mathscr{X}_i \in \mathbb{R}^{I_1\times I_2\times \cdots \times I_n }$, $i=1, \cdots, N$, threshold parameter $\tau$, kernel scaling parameter $\epsilon$, number of neighbors $K$, error tolerance $tot$ and max iterations $maxIter$
    \OUTPUT  MPS for tensor train subspace $\mathscr{U}_1, \mathscr{U}_2, \cdots, \mathscr{U}_n$
    \STATE Compute affinity matrix ${\bf S}$ by
    \[   {\bf S}_{ij} =\left\{
\begin{array}{ll}
      \exp(-\|\mathscr{X}_i -\mathscr{X}_j\|_F^2/ \epsilon), & \text{if } \mathscr{X}_{j: j\neq i} \in O(K, \mathscr{X}_i),\\
      0, & \text{otherwise},
\end{array} 
\right. \]

	\STATE Initialize $\mathscr{U}_{i:i=1,\cdots, n}$, ${\bf A}$ by TT-PCA algorithm and let $r_n $ be the number of rows in ${\bf A}$
	\STATE Form ${\bf D}\in \mathbb{R}^{I_1  \cdots  I_n\times N}$ as a reshape of the input data, and compute ${\bf Y} = {\bf D} -  {\bf D}{\bf S}^\top$
	\STATE Compute ${\bf Z} = {\bf Y} {\bf Y}^\top$
	\STATE Compute the eigenvectors of ${\bf Z}$ and set ${\bf V}_{r_n} $ to be the matrix of $r_n$ eigenvectors corresponding to the lowest eigenvalues. 
	
    	\STATE Set $iter =1$ %and $\mathscr{U} = \mathscr{U}_n$
    	\WHILE { $iter \leq maxIter$ or Convergence of ${\bf L}( \mathscr{U}_1 \cdots \mathscr{U}_n )$}
		 \FOR{ $i = 1$ to $n$}
		 	\STATE (Compute $\mathscr{T}_l$)
		 	\IF {$i=1$} \STATE $\mathscr{T}_l = {\bf I}$
			\ELSE \STATE Compute $\mathscr{T}_l = \mathscr{U}_1 \cdots \mathscr{U}_{i-1}$
			\ENDIF
			\STATE(Compute $\mathscr{T}_r$)
			\IF {$i=n$} \STATE $\mathscr{T}_r = {\bf I}$
			\ELSE \STATE Compute $\mathscr{T}_r = \mathscr{U}_{i+1} \cdots \mathscr{U}_{n}$
			\ENDIF
			\STATE Solve and update
			
			\begin{displaymath}
			\begin{split}
			\mathscr{U}_i =
			\argmin_{\substack{ \mathscr{U}_i : {\bf L}(\mathscr{U}_i)  \text{ is unitary}}} 
			&\| \left( {\bf I}_{I_i} \otimes {\bf L}(\mathscr{T}_l) \right) {\bf L}(\mathscr{U}_i) {\bf R}(\mathscr{T}_r) \\
			&-{\bf T}_i({\bf V}_{r_n})\|_F^2.
			\end{split}
			\end{displaymath}
			
			
			
			%\begin{displaymath}
			%\begin{split}
			%\mathscr{U}_i 
			%= \argmin_{\mathscr{U}_i:{\bf L}(\mathscr{U}_i)  \text{ is Unitary}} 		&\| \left( {\bf I}^{I_i} \otimes {\bf L}(\mathscr{T}_l) \right) {\bf L}(\mathscr{U}_i) {\bf R}					(\mathscr{T}_r) \\
			%&-\tilde{{\bf L}_i}^{-1}({\bf V}_{r_n})) \|_F^2
			%\end{split}
			%\end{displaymath}
			%\textcolor{red}{ Wenqi, try removing $\tilde{{\bf L}_i}^{-1}$}
		 \ENDFOR
		 
	%	 \IF{ $norm({\bf V}(\mathscr{U} - \mathscr{U}_n)) >= tot$ }
	%	 	$\mathscr{U}  = \mathscr{U}_n$
	%	\ELSE 
	%		\STATE Break
	%	\ENDIF
		
		\STATE $iter = iter +1 $
		 
	\ENDWHILE

\end{algorithmic}
\label{TTNPE-Algo}
\end{algorithm} 


==> Apdix.tex <==
\section{Appendix}
%\subsection{Proof for Lemma \ref{LemmaSP}}\label{ProofSP}
%(1) Let ${\bf a} = {\bf 0}$, then we know that ${\bf 0} \in {\bf S}_{TT}$
%
%(2) Let $\text{vec}(\mathscr{X}_1) ={\bf L}(\mathscr{U1}_1...\mathscr{U}_n) {\bf a}_1$, \text{vec}($\mathscr{X}_2) ={\bf L}(\mathscr{U1}_1...\mathscr{U}_n) {\bf a}_2$, then 
%\begin{equation}
%\text{vec}(\mathscr{X}_1) + \text{vec}(\mathscr{X}_2) = {\bf L}(\mathscr{U1}_1...\mathscr{U}_n) ({\bf a}_1 + {\bf a}_2) \in {\bf S}_{\text{TT}},
%\end{equation}
%thus we proof our claim.

\subsection{Proof for Lemma \ref{LemmaOP} }\label{ProofOP}
Theorem 1 in \cite{holtz2012manifolds} gives that $\forall_{i=1,\cdots, n} {\bf L}(\mathscr{U}_i)$ is a unitary matrix, thus we have ${\bf L}(\mathscr{U}_1)$ satisfies  \eqref{eq: OP}.  Assume ${\bf B}_j ={\bf L}(\mathscr{U}_1,\cdots, \mathscr{U}_{j})$ satisfies \eqref{eq: OP}, we have
\begin{equation}
{\bf B}_j^\top {\bf B}_j = {\bf I} \in \mathbb{R}^{r_j \times r_j}.
\end{equation}
Since ${\bf B}_{j+1} = {\bf L}(\mathscr{U}_1,\cdots, \mathscr{U}_{j+1}) = ({\bf I}^{I_{j+1}} \otimes {\bf B}_j) \times {\bf L}(\mathscr{U}_{j+1})$, thus we have
\[
\begin{split}
&{\bf B}_{j+1}^\top {\bf B}_{j+1} \\
=&({\bf L}(\mathscr{U}_{j+1}))^\top ({\bf I}^{I_{j+1}} \otimes {\bf B}_j)^\top ({\bf I}^{I_{j+1}} \otimes {\bf B}_j) \times {\bf L}(\mathscr{U}_{j+1}) \\
=&({\bf L}(\mathscr{U}_{j+1}))^\top
\begin{bmatrix}
{\bf B}_j^\top & \cdots & {\bf 0}\\
\vdots& \ddots & \vdots \\
{\bf 0}& \cdots & {\bf B}_j^\top
\end{bmatrix}
\begin{bmatrix}
{\bf B}_j & \cdots & {\bf 0}\\
\vdots& \ddots & \vdots \\
{\bf 0}& \cdots & {\bf B}_j
\end{bmatrix}
({\bf L}(\mathscr{U}_{j+1})) \\
=&({\bf L}(\mathscr{U}_{j+1}))^\top {\bf I} ({\bf L}(\mathscr{U}_{j+1})) \\
=& {\bf I} \in \mathbb{R}^{r_{j+1} \times r_{j+1}}.
\end{split}
\]
thus we proof our claim. 

==> Dim_Storage.tex <==
\section{Manifold Dimension  and Data Storage}
\subsection{PCA Model}
Under PCA model, a $I_1\cdots I_n$-dimensional data from rank-$r$ subspace can be represented by the linear combination of the $r$ bases vectors. Since the bases vectors are orthonormal with each other, Stiefel manifold shows that the manifold dimensional of the PCA model is
\begin{equation}
\mathbb{D}_{\text{PCA}} = (I_1\cdots I_n)r -\frac{1}{2} r(r+1)
\end{equation}
If there are $N$ data generated from the space, then the total storage for the $N$ given data is
\begin{equation}
\mathbb{S}_{\text{PCA}} = \mathbb{D}_{\text{PCA}} + rN
\end{equation}
where $rN$ stores the $N$ data. 

\subsection{Tucker-PCA (T-PCA) Model}
Under T-PCA model,  a tensor $\mathscr{T} \in \mathbb{R}^{I_1\times \cdots \times I_n}$ is represented by a compressed tensor $\mathscr{C} \in  \mathbb{R}^{r_1\times \cdots \times r_n}$, thus
\begin{equation}
\mathscr{C} = \mathscr{T} \times_1{\bf U}_1 \cdots \times_n {\bf U}_n
\end{equation}
where ${\bf U}_{i:i=1,..., n} \in \mathbb{R}^{r_i \times I_i}$.

The manifold dimensional is
\begin{equation}
\mathbb{D}_{\text{T-PCA}} = \sum_{i=1}^n (I_ir_i -r_i^2) + d\prod_{i=1}^n r_i
\end{equation}

%Thus, the manifold is the span of $\times_i {\bf U_i}, i=1,..., n$. Since the ${\bf U}_i$ may or may not be orthonormal matrix, thus the manifold dimension is
%\begin{equation}
%\mathbb{D}_{T-PCA} = \sum_{i=1}^n{I_i r_i}  + d\prod_{i=1}^n r_i \text{	(If not orthonormal)}
%\end{equation}
%and
%\begin{equation}
%\mathbb{D}_{T-PCA} = \sum_{i=1}^n{ \left( I_i r_i - \frac{1}{2}r_i(r_i+1) \right)} \text{	(If orthonormal)}
%\end{equation}

If there are $N$ data generated from the space, then the total storage for the $N$ given data is
\begin{equation}
\mathbb{S}_{\text{T-PCA}} =\sum_{i=1}^n (I_ir_i -r_i^2)+N \prod_{i=1}^n r_i
\end{equation}

\subsection{Tensor Train PCA (TT-PCA) Model}
Under Tensor Train PCA (TT-PCA) model,   a tensor $\mathscr{T} \in \mathbb{R}^{I_1 \times \cdots \times I_n}$ is represented by a vector ${\bf a} \in \mathbb{R}^{r_n \times 1}$, thus
\begin{equation}
\mathscr{T} = \mathscr{U}_1\cdots \mathscr{U}_n {\bf a}
\end{equation}
where $\mathscr{U}_i \in \mathbb{R}^{ r_{i-1} \times I_i \times r_i}$. 

The manifold dimension of tensor train model is 
\begin{equation}
\mathbb{D}_{\text{TT-PCA}}  = \sum_{i=1}^n r_{i-1}I_ir_i - \sum_{i=1}^{n-1} r_i^2
\end{equation}

If there are $N$ data generated from the space, then the total storage for the $N$ given data is
\begin{equation}
\mathbb{S}_{\text{TT-PCA}} = \mathbb{D}_{\text{TT-PCA}}  + Nr_n
\end{equation}


==> Lemma_SubspaceProperty.tex <==
{\lemma (Subspace Property) Tensor Train Subspace satisfies the following subspace property\\
(1) ${\bf 0} \in \mathscr{S}_{TT}$ \\
(2) If $\mathscr{X}_1 \in \mathscr{S}_{TT}$ and $\mathscr{X}_2 \in \mathscr{S}_{TT}$, then $\mathscr{X}_1 + \mathscr{X}_2 =\mathscr{X}_3 \in \mathscr{S}_{TT}$
}

{\proof
(1) Let ${\bf a} = {\bf 0}$, then we know that ${\bf 0} \in \mathscr{S}_{TT}$

(2) Let $\mathscr{X}_1 =\mathscr{U1}_1...\mathscr{U}_n {\bf a}_1$, $\mathscr{X}_2 =\mathscr{U1}_1...\mathscr{U}_n {\bf a}_2$ and let $\mathscr{X}_3 \in \mathscr{S}_{TT}$. Without loss of generality, we consider the $i_1,..., i_n$ entry in $\mathscr{X}_3$, which gives
\begin{equation}
\begin{split}
\mathscr{X}_3(i_1,..., i_n) &= \mathscr{X}_1(i_1,..., i_n)+ \mathscr{X}_2(i_1,..., i_n)\\
& = \mathscr{U}_1(:, i_1,:)...\mathscr{U}_n(:, i_n,:) {\bf a}_1(:, 1) \\
& + \mathscr{U}_1(:, i_1,:)...\mathscr{U}_n(:, i_n,:) {\bf a}_2(:, 1) \\
& = \mathscr{U}_1(:, i_1,:)...\mathscr{U}_n(:, i_n,:)({\bf a}_1(:, 1) + {\bf a}_2(:, 1)) \\
& = \mathscr{U}_1(:, i_1,:)...\mathscr{U}_n(:, i_n,:){\bf a}_3(:, 1),
\end{split}
\end{equation}
where ${\bf a}_3 ={\bf a}_1+ {\bf a}_2$. Thus $\mathscr{X}_3=\mathscr{U}_1...\mathscr{U}_n{\bf a}_3$, indicating that $\mathscr{X}_3 \in \mathscr{S}_{TT}$.
\endproof}

==> TNPE_Solver_Pre.tex <==
In order to solve this non-convex problem, we will use an Alternating Minimization Approach where in each iteration, we minimize w.r.t. each $\mathscr{U}_i$ keeping the rest as fixed. Thus, we only need to discuss how to minimize the above w.r.t. only one variable $\mathscr{U}_k$ when the rest are fixed. 

Let
\begin{equation}
\mathscr{T}_l = \mathscr{U}_1\cdots \mathscr{U}_{k-1} \in \mathbb{R}^{r_0 \times (I_1\cdots I_{k-1}) \times r_{k-1}} \quad
\end{equation}
and
\begin{equation}
\mathscr{T}_r = \mathscr{U}_{k+1}\cdots \mathscr{U}_{n} \in \mathbb{R}^{r_{k} \times (I_{k+1}\cdots I_{n}) \times r_{n}},
\end{equation}
thus $ {\bf L}(\mathscr{U}_1 \cdots \mathscr{U}_n )  = {\bf L}(\mathscr{T}_l \mathscr{U}_k \mathscr{T}_r)$.
Thus, the problem for optimizing over a single $\mathscr{U}_k$ becomes
\begin{equation}\label{eq: TTNPE6}
\min_{\substack{ \mathscr{U}_k: {\bf L}(\mathscr{U}_k)  \text{ is unitary}}} 
\|{\bf L}(\mathscr{T}_l \mathscr{U}_k \mathscr{T}_r)-{\bf V}_{r_n}\|_F^2.
\end{equation}


%Let
%\begin{equation}
%\mathscr{T}_l = \mathscr{U}_1\cdots \mathscr{U}_{k-1} \in \mathbb{R}^{r_0 \times (I_1\cdots I_{k-1}) \times r_{k-1}} \quad
%\end{equation}
%and
%\begin{equation}
%\mathscr{T}_r = \mathscr{U}_{k+1}\cdots \mathscr{U}_{n} \in \mathbb{R}^{r_{k} \times (I_{k+1}\cdots I_{n}) \times r_{n}},
%\end{equation}
%thus $ {\bf L}(\mathscr{U}_1 \cdots \mathscr{U}_n )  = {\bf L}(\mathscr{T}_l \mathscr{U}_k \mathscr{T}_r)$.
%\eqref{eq: TTNPE5} becomes
%\begin{equation}\label{eq: TTNPE6}
%\mathscr{U}^*_k = \argmin_{\mathscr{U}_k: {\bf L}(\mathscr{U}_k) \in \text{Unitary}} \| {\bf L}( \mathscr{T}_l \mathscr{U}_k \mathscr{T}_r ) - {\bf V}_{r_n}\|_F^2.
%\end{equation}
%%Note that $\mathscr{T}_l \mathscr{U}_k \mathscr{T}_r  \in \mathbb{R}^{1 \times (I_1\cdots I_n) \times r_n}$ and ${\bf V}_{r_n} \in \mathbb{R}^{(I_1\cdots I_n) \times r_n}$.

%The trick in solving \eqref{eq: TTNPE6} is that by introducing an artificial left refolding such that \eqref{eq: TTNPE6} can be solved by least square method. 
%Since the left refolding operator does not change Frobenius norm, let $\tilde{\bf L}^{-1}$ be the artificial left refolding operator and \eqref{eq: TTNPE6} becomes
%\begin{equation} \label{eq: TTNPE7.5}
%\begin{split}
%\mathscr{U}^*_k = \argmin_{\mathscr{U}_k: {\bf L}(\mathscr{U}_k) \in \text{Unitary}} &\| \tilde{\bf L}_k^{-1}\left( {\bf L}( \mathscr{T}_l \mathscr{U}_k \mathscr{T}_r ) \right) \\
%&- \tilde{\bf L}_k^{-1}({\bf V}_{r_n})\|_F^2 
%%& = \argmin_{\mathscr{U}_k:{\bf L}(\mathscr{U}_k) \in \text{Unitary}} 		\| \left( {\bf I}^{I_k} \otimes {\bf L}(\mathscr{T}_l) \right) {\bf L}(\mathscr{U}_k) {\bf R}(\mathscr{T}_r) -{\bf V}) \|_F^2
%\end{split}
%\end{equation}
%The $\tilde{{\bf L}_k}^{-1}$ operator gives
%\begin{equation} \label{eq: TTNPE7}
%\tilde{\bf L}_k^{-1}({\bf V}_{r_n}) = {\bf V} \in \mathbb{R}^{(I_1\cdots I_k) \times (I_{k+1} \cdots I_n) \times r_n},
%\end{equation}
%and
%\begin{equation}
%\tilde{\bf L}_k^{-1}\left( {\bf L}( \mathscr{T}_l \mathscr{U}_k \mathscr{T}_r ) \right)= \left( {\bf I}^{I_k} \otimes {\bf L}(\mathscr{T}_l) \right) {\bf L}(\mathscr{U}_k) {\bf R}(\mathscr{T}_r).
%\end{equation}
%
%thus \eqref{eq: TTNPE7.5} becomes

The problem in \eqref{eq: TTNPE6} can be solved by separating $\mathscr{T}_l, \mathscr{U}_k, \mathscr{T}_r$ into 3 matrices, 

The problem in \eqref{eq: TTNPE6}
Since reshape does not change the Frobenius norm of a tensor and Reshaping tensors does not changeThe problem in \eqref{eq: TTNPE6} can be solved by 


reduces to \textcolor{red}{Wenqi, please check. What is ${\bf V}$ - use another notation and do not use artificial things and define this precisely. }
\begin{equation} \label{eq: TTNPE8}
\begin{split}
\mathscr{U}^*_k 
= \argmin_{\mathscr{U}_k:{\bf L}(\mathscr{U}_k)  \text{ is Unitary}} 		&\| \left( {\bf I}^{I_k} \otimes {\bf L}(\mathscr{T}_l) \right) {\bf L}(\mathscr{U}_k) {\bf R}(\mathscr{T}_r) \\
&-{\bf V} \|_F^2.
\end{split}
\end{equation}
%where ${\bf R}(\mathscr{T}_r)  = (\mathscr{T}_r)_{[1]}$. 
This problem can be solved by the optimization algorithm for a differentiable function with unitary constraints as proposed in \cite{wen2013feasible}.  In the optimization, we can use that the gradient of $ \|{\bf A}{\bf X}{\bf B} - {\bf C}\|_F^2$ is ${\bf A}^\top ({\bf A}{\bf X}{\bf B}-{\bf C}){\bf B}^\top$. This algorithm, denoted TT-NPE, is described in Algorithm \ref{TTNPE-Algo}.

%Now \eqref{eq: TTNPE8} is a least square problem under unitary constraint, which can be solved by the optimization algorithm as proposed in \cite{wen2013feasible}, where the gradient is given by Lemma \ref{Gradient}. The details of the TT-NPE algorithm is described in \ref{TTNPE-Algo}

%{\lemma (Gradient) \label{Gradient}
%Let ${\bf A} \in \mathbb{R}^{n_1 \times r_1}, {\bf X} \in \mathbb{R}^{r_1\times r_2}, {\bf B} \in \mathbb{R}^{r_2 \times n_2}$ and ${\bf C}\in \mathbb{R}^{n_1\times n_2}$, then we have
%\begin{equation}
%\frac{\partial \|{\bf A}{\bf X}{\bf B} - {\bf C}\|_F^2}{\partial {\bf X}} = {\bf A}^\top ({\bf A}{\bf X}{\bf B}-{\bf C}){\bf B}^\top
%\end{equation}
%}

==> TT-NPE.tex <==
%\vspace{-.1in}
\section{Tensor Train Neighborhood Preserving Embedding (TT-NPE)} \label{NPE}
%\vspace{-.1in}

Given a set of tensor data $\mathscr{X}_{i}\in \mathbb{R}^{I_1 \times \cdots \times I_n}$,  $i=1,\cdots, N$, we wish to project the data  $\mathscr{X}_{i}$ to vector ${\bf t}_i \in \mathbb{R}^{r_n}$ using a Tensor Train embedding, satisfying ${\bf t}_i  =({\bf L}(\mathscr{U}_1 \cdots \mathscr{U}_n))^T {\bf V}(\mathscr{X}_{i}) $, and tries to preserve the distance in the projected data. In this Section, we use the objective function similar to that given in \cite{dai2006tensor} for Tucker embedding, and give an embedding for Tensor Train Decomposition. 





%Given a set of tensor data $\mathscr{X}_{i:i=1,\cdots, N} \in \mathbb{R}^{I_1 \times \cdots \times I_n}$, TT-NPE aims at finding a set of MPE to embed a tensor $\mathscr{X}_i \in \mathbb{R}^{I_1 \times \cdots \times I_n} $ into a vector ${\bf t}_i \in \mathbb{R}^{r_n \times 1}$ such that the local topological structure is preserved  and the geometric property is effectively captured.

  
%Our proposed TT-NPE applies the embedding merit given by \cite{dai2006tensor}, where representing a tensor by the affine combination of its close neighbors guarantees the geometry preserving property.   

We first construct a neighbor graph $G$ to capture the neighbor structure in the original given tensor space and  generate the affinity matrix ${\bf S}$ as
\[   {\bf S}_{ij} =\left\{
\begin{array}{ll}
      \exp(-\|\mathscr{X}_i -\mathscr{X}_j\|_F^2/ \epsilon), & \text{if } \mathscr{X}_{j: j\neq i} \in O(K, \mathscr{X}_i),\\
      0, & \text{otherwise},
\end{array} 
\right. \]
where $O(K, \mathscr{X}_i)$ denotes the sub-set of data excluding $\mathscr{X}_i$ that are within the $K$-nearest neighbor of $\mathscr{X}_i$, and $\epsilon$ is the scaling factor. By definition, ${\bf S}_{ii}=0$. We note that label information, even if available,  is not used to construct the affinity graph.

The goal is to find the decomposition $\mathscr{U}_1, \cdots, \mathscr{U}_n$ that minimize the average distance between the point and the weighted combination of other points which are weighted by the affinity matrix in the projection. More formally, we wish to find a solution for

\vspace{-.15in}
\begin{equation}\label{eq: TTNPE1}
\begin{split}
 &\min_{\substack{ \mathscr{U}_i \forall {i=1,\cdots, n}\\ {\bf L}(\mathscr{U}_i)  \text{ is Unitary}}}
\sum_i \|{\bf L}^\top( \mathscr{U}_1 \cdots \mathscr{U}_n ){\bf V}(\mathscr{X}_i )\\
&- \sum_j {\bf S}_{ij} {\bf L}^\top(\mathscr{ U}_1 \cdots \mathscr{U}_n ){\bf V}(\mathscr{X}_j)\|_2^2.
\end{split}
\end{equation}
\vspace{-.15in}
 
 Let ${\bf D}\in \mathbb{R}^{I_1  \cdots  I_n\times N}$ be the matrix that concatenates the $N$ vectorizations such that the $i^{\text{th}}$ column of ${\bf D}$ is  ${\bf V}({\mathscr{X}}_i)$. Then,  \eqref{eq: TTNPE1} can be reduced to 


%Let ${\bf x}_{i:i=1,\cdots, N} \in \mathbb{R}^{(I_1 \cdots I_n) \times 1}$ be the vectorized tensor data $\mathscr{X}_i$, ${\bf x}_i = {\bf V}(\mathscr{X}_i)$, 
%and ${\bf L}(\mathscr{U}_1 \cdots \mathscr{U}_n) \in \mathbb{R}^{(I_1\cdots I_n) \times r_n}$ be the tensor train subspace bases. 
%The goal is find a set of MPS such that following distance preservation problem is minimized
%\begin{equation}\label{eq: TTNPE1}
%\begin{split}
%&\min \sum_i \| {\bf t}_i - \sum_j {\bf S}_{ij} {\bf t}_j\|_2^2\\
% = &\min_{\substack{\forall_{i=1,\cdots, n} \mathscr{U}_i \\ {\bf L}(\mathscr{U}_i) \in \text{Unitary}}}
%\sum_i \|{\bf L}^\top( \mathscr{U}_1 \cdots \mathscr{U}_n ){\bf x}_i \\
%&- \sum_j {\bf S}_{ij} {\bf L}^\top(\mathscr{ U}_1 \cdots \mathscr{U}_n ){\bf x}_j\|_2^2
%\end{split}
%\end{equation}

%The equation \eqref{eq: TTNPE1} is further reduced to matrix forms for analysis, which gives
\vspace{-.1in}
\begin{equation}\label{eq: TTNPE2}
\begin{split}
%&\min_{\substack{\forall_{i} \mathscr{U}_i : {\bf L}(\mathscr{U}_i) \in \text{Unitary}}}
%\sum_i \|{\bf L}^\top( \mathscr{U}_1 \cdots \mathscr{U}_n )
%\left({\bf x}_i -  ({\bf x}_1, \cdots, {\bf x}_N)
%\left[\begin{matrix}
%{\bf S}_{i1}\\
%\vdots\\
%{\bf S}_{iN}
%\end{matrix}\right]
%\right)
%\|_2^2\\
\min_{\substack{ \mathscr{U}_i \forall {i=1,\cdots, n}\\ {\bf L}(\mathscr{U}_i)  \text{ is Unitary}}} 
\|{\bf L}^\top( \mathscr{U}_1 \cdots \mathscr{U}_n )({\bf D} -  {\bf D}{\bf S}^\top)\|_F^2.
\end{split}
\vspace{-.1in}
\end{equation}


%where ${\bf X } = [{\bf x}_1, \cdots, {\bf x}_n]$.
Since ${\bf D} -  {\bf D}{\bf S}^\top \in \mathbb{R}^{(I_1\cdots I_n) \times N}$ is known,  we set ${\bf Y} = {\bf D} -  {\bf D}{\bf S}^\top$.  The Frobenius norm in \eqref{eq: TTNPE2} can be further expressed in the form of matrix trace to reduce the problem to
\vspace{-.1in}
\begin{equation}\label{eq: TTNPE3}
%\min_{\substack{\forall_{i=1,\cdots, n} \mathscr{U}_i \\ {\bf L}(\mathscr{U}_i) \in \text{unitary}}} 		\|{\bf L}^\top( \mathscr{U}_1 \cdots \mathscr{U}_n ){\bf Y}\|_F^2=
\min_{\substack{ \mathscr{U}_i  \forall {i=1,\cdots, n}\\ {\bf L}(\mathscr{U}_i)  \text{ is unitary}}} 	\text{tr}  ( {\bf Y}^\top {\bf L}(\mathscr{U}_1 \cdots \mathscr{U}_n ) {\bf L}^\top( \mathscr{U}_1 \cdots \mathscr{U}_n ){\bf Y}) .
\vspace{-.1in}
\end{equation}


Based on the cyclic permutation property of trace operator, \eqref{eq: TTNPE3} is equivalent to 
\vspace{-.1in}
\begin{equation}\label{eq: TTNPE3_5}
%\min_{\substack{\forall_{i=1,\cdots, n} \mathscr{U}_i \\ {\bf L}(\mathscr{U}_i) \in \text{unitary}}} 		\|{\bf L}^\top( \mathscr{U}_1 \cdots \mathscr{U}_n ){\bf Y}\|_F^2=
\min_{\substack{\mathscr{U}_i \forall {i=1,\cdots, n}  \\ {\bf L}(\mathscr{U}_i)  \text{ is unitary}}} 	\text{tr}  ( {\bf L}^\top( \mathscr{U}_1 \cdots \mathscr{U}_n ){\bf Y} {\bf Y}^\top {\bf L}(\mathscr{U}_1 \cdots \mathscr{U}_n )  ). 
\vspace{-.1in}
\end{equation}


Let ${\bf Z} = {\bf Y} {\bf Y}^\top \in \mathbb{R}^{(I_1\cdots I_n) \times (I_1\cdots I_n)}$ be the constant matrix, and let us denote ${\bf E}= {\bf L}( \mathscr{U}_1 \cdots \mathscr{U}_n )$. Then, the problem reduces to 
\vspace{-.15in}
\begin{equation}\label{eq: TTNPE4}
%\min_{\substack{\forall_{i=1,\cdots, n} \mathscr{U}_i \\ {\bf L}(\mathscr{U}_i) \in \text{unitary}}} 	\text{tr}  (  {\bf L}^\top( \mathscr{U}_1 \cdots \mathscr{U}_n ){\bf Y} {\bf Y}^\top  {\bf L}(\mathscr{U}_1 \cdots \mathscr{U}_n )) = 
\min_{\substack{\mathscr{U}_i \forall {i=1,\cdots, n} \\ {\bf L}(\mathscr{U}_i)  \text{ is unitary}}} 	 \text{tr}  (  {\bf E}^\top{\bf Z} {\bf E}) .
\end{equation}
\vspace{-.15in}

We note that the solution to minimize the quadratic form  $ \text{tr}  (  {\bf E}^\top{\bf Z} {\bf E}) $ where ${\bf E}$ is unitary is given by ${\bf E}$ being the matrix formed by eigenvectors corresponding to the lowest eigenvalues of ${\bf Z}$ and the value of the objective is the sum of the lowest eigen-values of ${\bf Z}$ \cite{moslehian2012ky}. Let the matrix corresponding to the eigenvectors corresponding to $r_n$ least eigenvalues of ${\bf Z}$ be ${\bf V}_{r_n}$. 
The solution so far does not account that ${\bf E}$ is formed by TT decomposition. With the additional constraint that ${\bf E}$ has TT decomposition, the above choice of ${\bf E}$ may not be optimal. 
%With the additional constraints that each $\mathscr{U}_i $ is unitary, this value of ${\bf E}$ may not be achievable. 
Thus, we relax the original problem to minimize the distance between ${\bf E}$ and ${\bf V}_{r_n}$. Thus, the relaxed problem is 

%The minimization in \eqref{eq: TTNPE4} indicates ${\bf L}(\mathscr{U}_1 \cdots \mathscr{U}_n )$ are the eigenvectors corresponding to the smallest $r_n$ eigenvalues of ${\bf Z}$, denoted as ${\bf V}_{r_n}$. Thus the relaxed problem of  \eqref{eq: TTNPE4} becomes

\vspace{-.1in}
\begin{equation}\label{eq: TTNPE5}
\min_{\substack{ \mathscr{U}_i \forall {i=1,\cdots, n} \\ {\bf L}(\mathscr{U}_i)  \text{ is unitary}}} 
\| {\bf L}(\mathscr{U}_1 \cdots \mathscr{U}_n ) -{\bf V}_{r_n}\|_F^2,
\vspace{-.1in}
\end{equation}
where ${\bf L}(\mathscr{U}_1 \cdots \mathscr{U}_n), {\bf V}_{r_n} \in \mathbb{R}^{(I_1 \cdots I_n) \times r_n}$. 

An Alternating Minimization method is proposed to solve \eqref{eq: TTNPE5}, where each $\mathscr{U}_{k:k=1,\cdots, n}$ is updated keeping rest fixed. Without loss of generality, we formulate the optimization problem for solving $\mathscr{U}_k$ when the rest are fixed, thus the problem for updating for $\mathscr{U}_k$ is
\vspace{-.1in}
\begin{equation}\label{eq: TTNPE10}
\min_{\substack{ \mathscr{U}_k : {\bf L}(\mathscr{U}_k)  \text{ is unitary}}} 
\| {\bf L}(\mathscr{U}_1 \cdots \mathscr{U}_n ) - {\bf V}_{r_n}\|_F^2.
\vspace{-.1in}
\end{equation}

Let ${\bf T}_i$ be a reshaping operator that change the dimension of a matrix from $\mathbb{R}^{(I_1\cdots I_n) \times r_n}$ to $\mathbb{R}^{(I_1 \cdots I_i) \times (I_{i+1}\cdots I_n r_n)}$, thus \eqref{eq: TTNPE10} becomes
\vspace{-.1in}
\begin{equation}\label{eq: TTNPE9}
\min_{\substack{ \mathscr{U}_k : {\bf L}(\mathscr{U}_k)  \text{ is unitary}}} 
\| {\bf T}_k({\bf L}(\mathscr{U}_1 \cdots \mathscr{U}_n )) - {\bf T}_k({\bf V}_{r_n})\|_F^2.
\vspace{-.1in}
\end{equation}


Let
\vspace{-.1in}
\begin{equation}
\mathscr{T}_l = \mathscr{U}_1\cdots \mathscr{U}_{k-1} \in \mathbb{R}^{r_0 \times (I_1\cdots I_{k-1}) \times r_{k-1}} \quad
\vspace{-.1in}
\end{equation}
and
\vspace{-.1in}
\begin{equation}
\mathscr{T}_r = \mathscr{U}_{k+1}\cdots \mathscr{U}_{n} \in \mathbb{R}^{r_{k} \times (I_{k+1}\cdots I_{n}) \times r_{n}},
\vspace{-.1in}
\end{equation}
then \eqref{eq: TTNPE9} becomes
\vspace{-.1in}
\begin{equation}\label{eq: TTNPE11}
\min_{\substack{ \mathscr{U}_k: {\bf L}(\mathscr{U}_k)  \text{ is unitary}}} 
\| {\bf T}_k({\bf L}(\mathscr{T}_l \mathscr{U}_k \mathscr{T}_r))-{\bf T}_k({\bf V}_{r_n})\|_F^2.
\vspace{-.1in}
\end{equation}

Since ${\bf T}_k({\bf L}(\mathscr{T}_l \mathscr{U}_k \mathscr{T}_r)) = \left( {\bf I}_{I_k} \otimes {\bf L}(\mathscr{T}_l) \right) {\bf L}(\mathscr{U}_k) {\bf R}(\mathscr{T}_r)$,
where ${\bf I}_{I_k}$ is an identity matrix of dimension $I_k$. 
The reshaping separates $\mathscr{T}_l, \mathscr{U}_k$ and $\mathscr{T}_r$ and \eqref{eq: TTNPE11} is reduced to
%$ {\bf I}^{I_k} \otimes {\bf L}(\mathscr{T}_l)  \in \mathbb{R}^{(I_1 \cdots I_k) \times (r_{k-1}I_k) }$, 
%${\bf L}(\mathscr{T}_l) \in \mathbb{R}^{ (r_{k-1}I_k) \times r_k} $,
%${\bf R}(\mathscr{T}_r) \in \mathbb{R}^{r_k \times (I_{k+1} \cdots I_nr_n)}$
%and ${\bf S}_k({\bf V}_{r_n}) \in \mathbb{R}^{(I_1\cdots I_k) \times (I_{k+1} \cdots I_nr_n)}$, 
\vspace{-.1in}
\begin{equation}\label{eq: TTNPE12}
\min_{\substack{ \mathscr{U}_k \\ {\bf L}(\mathscr{U}_k)  \text{ is unitary}}} 
\| \left( {\bf I}_{I_k} \otimes {\bf L}(\mathscr{T}_l) \right) {\bf L}(\mathscr{U}_k) {\bf R}(\mathscr{T}_r)-{\bf S}_k({\bf V}_{r_n})\|_F^2.
\vspace{-.1in}
\end{equation}

This problem can be solved by the optimization algorithm for a differentiable function with unitary constraints as proposed in \cite{wen2013feasible}.  
In the optimization, we can use that the gradient of $ \|{\bf A}{\bf X}{\bf B} - {\bf C}\|_F^2$ is ${\bf A}^\top ({\bf A}{\bf X}{\bf B}-{\bf C}){\bf B}^\top$. This algorithm, denoted TT-NPE, is described in Algorithm \ref{TTNPE-Algo}.
%\input{TNPE_Solver_Pre}
%Since tensor left refolding operator does not change the problem, we apply left refolding ${\bf L}^{-1} $ onto \eqref{eq: TTNPE5} and the equation becomes
%\begin{equation}
%\min_{\substack{ \mathscr{U}_i \forall {i=1,\cdots, n} \\ {\bf L}(\mathscr{U}_i)  \text{ is unitary}}} 
%\| \mathscr{U}_1 \cdots \mathscr{U}_n  -{\bf L}^{-1}({\bf V}_{r_n})\|_F^2,
%\end{equation}
%where ${\bf L}^{-1}({\bf V}_{r_n}),  \mathscr{U}_1 \cdots \mathscr{U}_n \in \mathbb{R}^{1 \times (I_1 \cdots  I_n) \times r_n}$.

%can be solved by tensor train decomposition \cite{oseledets2011tensor}


\input{Algo_TTNPE}
%\vspace{-.05in}

\subsection{Classification Using TT-NPE}
\vspace{-.05in}

The classification is conducted by first solving a set of MPS $\mathscr{U}_1 ,\cdots,\mathscr{U}_n$ by TT-NPE algorithm.
Then let ${\bf U} = {\bf L}(\mathscr{U}_1 \cdots \mathscr{U}_n)$ and embedding is conducted by projecting training data and testing data onto the bases ${\bf U}$. 
Any data point in the testing set $\mathscr{Y}\in \mathbb{R}^{I_1 \times \cdots \times I_n}$ is labeled by applying KNN classification with $K$ neighbors in the embedded space. 
\vspace{-0.1in}
\subsection{Storage and Computation Complexity}
In this section we will analyze the amount of storage to store the high dimensional data, complexity for doing TT-NPE and classification based on TT-NPE. 
KNN and TNPE \cite{dai2006tensor} algorithms are considered for comparison.  
For the computational complexity analysis, let $d$ be the data dimension, $n$ and $r$ be the tensor order and rank under TT-NPE model, $K$ be the number of neighbors and $N_{\text{tr}}\text{ }(N_{\text{te}})$ be the total training (testing) data. 

{\bf Storage of data: }
Under KNN model, the storage required for $N_{\text{tr}} $ training data is
$\text{Storage(KNN)} = dN_{\text{tr}}$.
%
Under TNPE model, the storage for the $N_\text{tr}$ training data needs the space for $n$ orthonormal linear transformation which is $n(d^{\frac{1}{n}} r -\frac{r(r+1)}{2})$, and the space for $N_\text{tr}$ embedded training data of size $N_\text{tr} r^n$, requiring the total storage 
$\text{Storage(TNPE)} =r^nN_{\text{tr}} + n(d^{\frac{1}{n}} r -\frac{r(r+1)}{2})$.
%
Under TT-NPE model, we need space $d^{\frac{1}{n}}r(r(n-1)+1) -\frac{r(r+1)n}{2}$ to store the projection bases $\mathscr{U}_1, \cdots, \mathscr{U}_n$, and $N_\text{tr} r_n$ to store the embedded training data. Thus the total storage is 
$\text{Storage(TT-NPE)} = d^{\frac{1}{n}}r(r(n-1)+1) -\frac{r(r+1)n}{2} + rN_\text{tr}$.

We consider a metric of normalized storage, {\em compression ratio}, which is the ratio of storage required under the embedding method and storage for the entire data, calculated by $\rho_{\text{ST}} = \frac{\text{Storage(ST)}}{N_\text{tr}d}$, where $\text{ST}$ can be any of KNN, TNPE, TT-NPE.

{\bf Computation Complexity for Embedding}
Under KNN model, data is directly used for classification and there is no embedding process. 
%
Under TNPE model, the embedding needs 3 steps, where solving $n$ linear transform takes $O(N_{\text{tr}}rd)$ for embedding raw data, 
matrix generation for an eigen-value problem takes $O(N_{\text{tr}}r^{2n})$, 
and eigenvalue decomposition for updating each linear transform takes $r^{3n}$, 
giving a total computational complexity $O(n(N_{\text{tr}}rd +N_{\text{tr}}r^{2n} + r^{3n}))$.
%
Under TT-NPE model, the embedding takes 4 steps, where 
the initialization by TT-PCA algorithm takes $O(nd^{\frac{1}{n}}r^3)$,
the generation of ${\bf Z}$ takes $O(d^2N_\text{tr})$,
solving ${\bf V}_{r_n}$ takes $O(d^3)$,
and updating $\mathscr{U}_k$ by solving a least square problem under unitary constraint takes $O(d^{\frac{1}{n}} r^3)$ \cite{wen2013feasible},
giving a total computational complexity $O(nd^{\frac{1}{n}}r^3 + d^2N_\text{tr} + d^3 + nd^{\frac{1}{n}} r^3)$.

{\bf Classification Complexity}
Under KNN model, classification is conducted by pair-wise computations of the distance between a testing point with all training points, which has a computational complexity of $O(N_{\text{te}}  N_{\text{tr}} d)$.
%
Under TNPE model, an extra time is required for embedding the testing data, which is  $O(r^2d N_{\text{te}})$. However less time is needed in classification by applying KNN in a reduced dimension, which is $O(N_{\text{tr}}N_{\text{te}}r^n)$. Thus the total complexity is $O(r^2dN_{\text{te}} + N_{\text{tr}}N_{\text{te}}r^n)$.
%
Similarly, under TT-NPE algorithm, embedding takes an extra computation time of  $O(N_\text{te}r^2d)$, but a significantly less time used in classification, which is $O(N_\text{te}N_\text{tr}r)$. Thus the total complexity is  $O(N_\text{te}r^2d + N_\text{te}N_\text{tr}r)$.

The comparison of the three algorithm is shown in Table \ref{ComplexityTable2}, where TT-NPE algorithm shows a great advantage in storage and computation for classification after embedding. 


\begin{table*}[t!]
  \centering
  \scalebox{0.8}{
  \begin{tabular}{cccc}
    \toprule
    & Storage & Subspace Computation & Classification\\
    \midrule
    KNN	&  $dN_{\text{tr}} $										& ${\bf 0}$ 												& $O(N_{\text{te}}  N_{\text{tr}} d)$\\
    TNPE	&  $r^nN_\text{tr} + n(d^{\frac{1}{n}}r -\frac{r(r+1)}{2})$ 					& $O(n(N_\text{tr}rd + N_\text{tr}r^{2n} + r^{3n}))$ 								& $O(N_{\text{te}}r^2d + N_{\text{te}}N_{\text{tr}}r^n)$\\
    TT-NPE&  ${\bf d^{\frac{1}{n}}r(r(n-1)+1) -\frac{r(r+1)n}{2} + rN_\text{tr}}$ 	& $O(nd^{\frac{1}{n}}r^3 + d^2N_\text{tr} + d^3 + nd^{\frac{1}{n}} r^3)$ 	& ${\bf O(N_\text{te}r^2d + N_\text{te}N_\text{tr}r)}$\\
    \bottomrule
  \end{tabular}
  }
   \label{ComplexityTable2}
  \caption{\small Storage and Computation Complexity Analysis for  Embedding Methods. The bold entry in each column depicts the lowest order. }
  \vspace{-.2in}
\end{table*}






==> YaleFace_Section_TBR.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% YaleFace %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-.1in}
\subsection{YaleFace Dataset}
\begin{figure}[t!]
\includegraphics [trim=0.5in 2.6in 1in 2.8in, keepaspectratio, width=0.4\textwidth] {YaleFace_Clusters_updated}
\centering
\vspace{-.1in}
\caption{Clustering Error Versus Number of Persons in YaleFace Dataset.}
\label{simu_YALE}
\vspace{-.1in}
\end{figure}

%Our motivation for applying polyhedral cones algorithm to cluster human faces is that human faces under different illuminations have been shown to be from union of polyhedral cones and each faces corresponds to a polyhedral cone respectively.

We will now evaluate the performance of KNN-SC algorithm in clustering human faces from the Extended Yale B data set \cite{georghiades2001few, lee2005acquiring}. We resize the images to  $48 \times 42$ pixels for ease of calculation. YaleFace includes the faces of $38$ persons with $64$ faces for each person. 
We choose 
%\textcolor{red}{What is $U \rightarrow$} 
$U$ out of $38$ people uniformly at random and depict the comparisons of different algorithms for varying values of $U$ from two to eight in 
%\textcolor{red}{This is Figure 5 - always label the Figs and use the ref command $\rightarrow$} 
Figure \ref{simu_YALE}.  For each point plotted, the clustering error is the average of $20$ random choices of selecting $U$ persons. We note that NCL and LSA algorithms are comparable, and perform the best when number of persons selected is small. The clustering error increases as the number of persons ($U$) increases, and KNN-SC performs the best for $U>5$. Beyond $U=6$, there is more than $10\%$ gap between the performance of KNN-SC with $K=2$ and Gaussian Kernels and the LSA/NCL algorithms.


%randomly sampled instances generated by the uniform sampling from the 38 persons. NCL algorithm performs  comparable with LSA algorithm and the two algorithms have shown the best performance for binary clustering, where the clustering error is 2\%. 
%However, the clustering error increases fast when number of clusters increases. In contrast, KNN-SC algorithm shows relative stable performance when the number of persons increases. KNN-SC with gaussian kernels show the best performance when the number of persons selected are more than 6, where the clustering for KNN-SC is less than 20\% as compared with 30\% for NCL algorithm.

==> simu_TTNPE.tex <==
\subsection{TT-NPE on MNIST Dataset}

In this subsection, we compare the proposed  tensor train neighbor preserving embedding (TT-NPE) algorithm with Tucker decomposition based  neighbor preserving embedding (TNPE) algorithm as proposed in \cite{dai2006tensor}. We use the MNIST dataset \cite{lecun1998gradient}, which consists 60000 of handwritten digits from $0$ to $9$. We select digits $1$ and $2$  for binary classification. $1000$ noiseless images for each digit are selected at random for training, and another $1000$ noiseless images are selected for testing. 


%In this section we compared our proposed tensor train neighbor preserving embedding (TT-NPE) algorithm with tensor neighbor preserving embedding (TNPE) algorithm as proposed in \cite{dai2006tensor}. The TNPE algorithm is selected as it shows the best performance  for tensor embedding when the label information is not available. 

%In the numerical result, MNIST dataset \cite{lecun1998gradient} that consists 60000 images of handwritten digits from 0 to 9 is selected. For ease of calculation, digits 1 and 2 are selected for binary classification. 1000 noiseless images from each digit are selected for training and another out of sample 1000 noiseless images are selected for testing.  
\begin{figure}[t!]
%\includegraphics [trim=.1in 2.6in 1in 2.2in, keepaspectratio, width=0.22\textwidth] {C2_Tr1000_Te1000_K1}
\includegraphics [trim=.1in 2.6in 1in 2.2in, keepaspectratio, width=0.22\textwidth] {C2_Tr1000_Te1000_K5}
\includegraphics [trim=.1in 2.6in 1in 2.2in, keepaspectratio, width=0.22\textwidth] {C2_Tr1000_Te1000_K10}
\centering
%\vspace{-.1in}
\caption{\small Classification Error in $\log10$ scale for MNIST under KNN, TNPE and TT-NPE model.  1000  images for each of digits 1, 2 are selected for training, and another  1000 noiseless images are selected for testing. The figure depicts the performance for the number of neighbors $K=5$ and $K=10$ respectively. }
\label{TTNPE_MNIST}
\vspace{-.25in}
\end{figure}


\textbf{Classification using TT-NPE} - Figure \ref{TTNPE_MNIST} shows the performance of the three algorithms (KNN on data directly, TNPE, and TT-NPE) for different values of $K = 5, 10$. Since KNN does not compress the data, it results in a single point at compression ratio of $1$. We note that the proposed TT-NPE is the same as the standard KNN for that point. Further, as the compression ratio increases, the classification error of the proposed TT-NPE decreases first, since TT-NPE model can  effectively capture of the embedded data structure. The  classification then increases since it fits the inherent noise as compared to the low TT-rank approximation of the data. \emph{Overall, TT-NPE algorithm shows comparable embedding performance as TNPE algorithm in the compression ratio region lower than 0.4, and outperforms TNPE for higher compression ratios (lesser compression)}. %Thus, TT-NPE gives more flexibility of choosing different rank parameters, and a lower computational complexity as compared to TNPE motivating its use in practice.

%, indicating the more controllable  and adjustable ability in  parameter tuning as compared with TNPE algorithm. 

 
%The simulation result in Fig \ref{TTNPE_MNIST} shows that with the increasing of the compression ratio, the classfication error of the proposed TT-NPE decreases first, which is caused by the effectively capture of the embedded data structure. 
%Then the classification increases and it is causes by the fitting of the noise in the given data which drifts the embedded structure away from the ground truth. 
%As the the compression ration is close to 1, the embedded structure has less freedom and returns to the original data space. 
%Thus, at the compression ratio of 1, the proposed TT-NPE algorithm gives the same result as K-nearest-neightbor (KNN) algorithm. 
%Overall, TT-NPE algorithm shows comparable embedding performance as TNPE algorithm in the compression ratio region lower than 0.4 and outperforms TNPE in the remaining compression region. 
%Moreover, TT-NPE gives more flexibility in compression  ratio, indicating the more controllable  and adjustable ability in  parameter tuning as compared with TNPE algorithm. 
